Proximal algorithms for large-scale statistical modeling and sensor/actuator selection

Several problems in modeling and control of stochastically-driven dynamical systems can be cast as regularized semi-definite programs. We examine two such representative problems and show that they can be formulated in a similar manner. The first, in statistical modeling, seeks to reconcile observed statistics by suitably and minimally perturbing prior dynamics. The second seeks to optimally select a subset of available sensors and actuators for control purposes. To address modeling and control of large-scale systems we develop a unified algorithmic framework using proximal methods. Our customized algorithms exploit problem structure and allow handling statistical modeling, as well as sensor and actuator selection, for substantially larger scales than what is amenable to current general-purpose solvers. We establish linear convergence of the proximal gradient algorithm, draw contrast between the proposed proximal algorithms and alternating direction method of multipliers, and provide examples that illustrate the merits and effectiveness of our framework.

==> figures/Tikz_common_styles.tex <==
%_______________________________________________________________
%
%     Tikz_common_styles
%
%     TikZ styles for drawing block diagrams.
%
%      Roy Smith,  15 July 2014
%
%_______________________________________________________________
\typeout{Reading Tikz styles:  Tikz_common_styles}
%
%   Block diagram styles
\tikzstyle{block} = [draw,rectangle,thick,minimum height=2em,minimum width=1.0cm,
                                top color=blue!10, bottom color=blue!10]%
\tikzstyle{sum} = [draw,circle,inner sep=0mm,minimum size=2mm]%
\tikzstyle{connector} = [->,thick]%
\tikzstyle{line} = [thick]%
\tikzstyle{branch} = [circle,inner sep=0pt,minimum size=1mm,fill=black,draw=black]%
\tikzstyle{guide} = []%
%
%   colours for various blocks
\tikzstyle{deltablock} = [block, top color=red!10, bottom color=red!10]%
\tikzstyle{controlblock} = [block, top color=green!10, bottom color=green!10]%
\tikzstyle{weightblock} = [block, top color=orange!10, bottom color=orange!10]%
\tikzstyle{clpblock} = [block, top color=cyan!10, bottom color=cyan!10]%
%
%  styles for dimming block components.
\tikzstyle{block_dim} = [draw,rectangle,thick,minimum height=2em,minimum width=2em,
                                color=black!15]%
\tikzstyle{sum_dim} = [draw,circle,inner sep=0mm,minimum size=2mm,color=black!15]%
\tikzstyle{connector_dim} = [->,thick,color=black!15]%
%
%    Graph styles
\tikzstyle{smalllabel} = [font=\footnotesize]%
\tikzstyle{axiswidth}=[semithick]%
\tikzstyle{axiscolor}=[color=black!50]%
\tikzstyle{help lines} =[color=blue!40,very thin]%
\tikzstyle{axes} = [axiswidth,axiscolor,<->,smalllabel]%
\tikzstyle{axis} = [axiswidth,axiscolor,->,smalllabel]%
\tikzstyle{tickmark} = [thin,smalllabel]%
\tikzstyle{plain_axes} = [axiswidth,smalllabel]%
\tikzstyle{w_axes} = [axiswidth,->,smalllabel]%
\tikzstyle{m_axes} = [axiswidth,smalllabel]%
\tikzstyle{dataplot} = [thick]%
%
%_______________________________________________________________


==> figures/filter_linsys.tex <==
%_______________________________________________________________________________
%
%   tikz figure for inclusion in exercises:
%
%   clp_2dof_output_pert_config:  closed loop system with perturbed models.  This uses
%                                              and input perturbation and the 2-DOF structure used for
%                                              the satellite example.
%
%   Marcello Colombino, 4 May 2015
%  
%_______________________________________________________________________________
%
% TikZ styles for drawing
%
\input{figures/Tikz_common_styles}
%
%   set a filename for externalization
% \tikzsetnextfilename{clp_2dof_input_pert_config}
%
\noindent
\begin{tikzpicture}[scale=1, auto, >=stealth']
  
    \small

   % specify with respect to the plant
    
     \node[block, minimum height = .8cm, top color=RoyalBlue!20, bottom color=RoyalBlue!20] (sys1) {filter};
     
     \node[block, minimum height = 1cm, top color=RoyalBlue!20, bottom color=RoyalBlue!20] (sys2) at ($(sys1.east) + (2.4cm,0)$) {$\ba{c} \mbox{linear} \\ \mbox{system}\ea$};
     
     \node[] (output-node) at ($(sys2.east) + (1.6cm,0)$) {};
     
     \node[] (input-node) at ($(sys1.west) - (1.6cm,0)$) {}; 
      
%     \node[sum, anchor=west](usum) at ($(G.west) - (5.75cm,0)$) {+}; 
%     
%     \node[block, anchor=west] (delta) at ($(usum) + (0.5cm,0.75cm)$) {$\Delta(s)$};
%     
%     \node[block, anchor=east] (W) at ($(delta.east) + (2. 5cm,0cm)$) {$W_I(s)$}; 
%      
%     \node[block,  anchor=west ] (K) at ($(G.east) + (0.75cm,0)$) {$k$} ; 
%      
%     \node[branch] (ubranch) at ($(delta.east) + (3cm,-0.75cm)$) {};
%
%     \node [sum, anchor=west] (esum) at ($(ubranch) + (4.55cm,0)$) {$+$};
%      
%     \node[guide] (y) at ($(G.south) - (0,0.5cm)$){};
%
%     \node[guide] (R) at ($(esum.east) + (1,0.0cm)$){};

    % now link the nodes

    \draw [connector] (input-node) -- node [midway, above] {$\ba{c} \mbox{white} \\ \mbox{noise} \ea$} node [midway, below] {$d$} (sys1.west);
    \draw [connector] (sys2.east) -- node [midway, below] {$x$} (output-node);
    \draw [connector] (sys1.east) -- node [midway, above] {$\ba{c} \mbox{colored} \\ \mbox{noise} \ea$} node [midway, below] {$f$} (sys2.west);
%    \draw [connector] (W) --   node [midway, above] {$z$} (delta);
%    \draw [connector] (ubranch) |-  (W);
%    \draw [connector] (delta) -| node [midway, above] {$v$}  (usum);
%    \draw [connector] (G) -- (usum); 
%    \draw [connector] (usum) -- node [near end, above, yshift=6pt] {$y$} 
%                                   ($(ybranch)-(0.75cm,0)$);
%    \draw [line] (ybranch) |- (y.east);
%    \draw [connector] (y) -| node [pos=0.9, right]{$-$} (esum);
%    \draw [connector] (R) -- node[midway, above] {$r$} (esum);                                            
\end{tikzpicture}
%_______________________________________________________________________________


==> figures/linsys_feedback.tex <==
%_______________________________________________________________________________
%
%   tikz figure for inclusion in exercises:
%
%   clp_2dof_output_pert_config:  closed loop system with perturbed models.  This uses
%                                              and input perturbation and the 2-DOF structure used for
%                                              the satellite example.
%
%   Marcello Colombino, 4 May 2015
%  
%_______________________________________________________________________________
%
% TikZ styles for drawing
%
\input{figures/Tikz_common_styles}
%
%   set a filename for externalization
% \tikzsetnextfilename{clp_2dof_input_pert_config}
%
\noindent
\begin{tikzpicture}[scale=1, auto, >=stealth']
  
    \small

   % specify with respect to the plant
    
     \node[block, minimum height = .8cm, top color=RoyalBlue!20, bottom color=RoyalBlue!20] (sys1) {$\ba{c} \mbox{linear} \\ \mbox{system}\ea$};
     
     \node[block, minimum height = .8cm, top color=blue!10, bottom color=blue!10] (sys4) at ($(sys1.south) - (0cm,.8cm)$) {$K$};
     
     \node[] (input-node) at ($(sys1.west) - (3.6cm,0)$) {}; 
     
     \node[] (output-node) at ($(sys1.east) + (2.3cm,0)$) {};
     
     \node[] (mid-node1) at ($(sys1.east) + (1cm,1cm)$) {}; 
          
     \node[sum] (esum1) at ($(sys1.west) - (1.8cm,0)$) {$+$};
           
     \node[branch] (R) at ($(sys1.east) + (.7cm,0.0cm)$){};
     
    % now link the nodes
	
%    \draw[connector] (ybranch) -- ++(0,-1.25cm) -| node [very near end, right] {$-$} (esum.south);

%%    \draw [connector] (input-node) -- node [midway, above] {$\ba{c} \mbox{\tc{RoyalBlue}{white}} \\ \mbox{\tc{RoyalBlue}{noise}} \ea$} node [midway, below] {$\tc{RoyalBlue}{\bw}$} (esum.west);
%%    \draw [connector] (esum.east) -- node [midway, above] {$\ba{c} \mbox{\tc{red}{colored}} \\ \mbox{\tc{red}{noise}} \ea$} node [midway, below] {$\tc{red}{\bd}$} (sys1.west);
	
    \draw [connector] (input-node) -- node [midway, above] {$\ba{c} \mbox{white} \\ \mbox{noise} \ea$} node [midway, below] {$d$} (esum1.west);
                    	
    \draw [line] (sys1.east) -- (R);
    \draw [connector] (R.west) -- node [midway, below] {$x$} (output-node);
%    \draw [connector] (esum1.east) -- node [midway, below] {$\bv$} (output-node);
    
    \draw [connector] (R.south) |- (sys4.east);
    
    \draw [connector] (sys4.west) -| (esum1.south);
    
    \draw [connector] (esum1.east) -- node [midway, above] {$\ba{c} \mbox{colored} \\ \mbox{noise} \ea$} node [midway, below] {$f$} (sys1.west);
    
%    \draw [connector] (mid-node) -- -| (sys2.east)
    
%    \draw [connector] (W) --   node [midway, above] {$z$} (delta);
%    \draw [connector] (ubranch) |-  (W);
%    \draw [connector] (delta) -| node [midway, above] {$v$}  (usum);
%    \draw [connector] (G) -- (usum); 
%    \draw [connector] (usum) -- node [near end, above, yshift=6pt] {$y$} 
%                                   ($(ybranch)-(0.75cm,0)$);
%    \draw [line] (ybranch) |- (y.east);
%    \draw [connector] (y) -| node [pos=0.9, right]{$-$} (esum);
%    \draw [connector] (R) -- node[midway, above] {$r$} (esum);                                            
\end{tikzpicture}
%_______________________________________________________________________________


==> my_definitions.tex <==
\newcommand{\new}{{\rm new}}
\newcommand{\old}{{\rm old}}
\newcommand{\barp}{{\bar p}}
\newcommand{\Diag}{{\rm Diag}\;}
\newcommand{\CP}{{\cal P}}
\newcommand{\rmCAP}{{\rm CAP}}
\newcommand{\epc}{\hspace{1pc}}
\newcommand{\gap}{\vspace{0.1in}}
\newcommand{\Mbld}{{\mbox{\bf M}}}
\newcommand{\Xbld}{{\mbox{\bf X}}}
\newcommand{\qbld}{{\mbox{\bf q}}}
\newcommand{\scmax}{{\rm {\scriptstyle max}}}
\newcommand{\scdia}{{\rm {\scriptstyle dia}}}
\newcommand{\sclow}{{\rm {\scriptstyle low}}}
\newcommand{\scupp}{{\rm {\scriptstyle upp}}}
\newcommand{\thalf}{{\textstyle \frac{1}{2}}}
\newcommand{\cA}{{\cal A}}
\newcommand{\cl}{{\cal L}}
\newcommand{\cC}{{\cal C}}
\newcommand{\cD}{{\cal D}}
\newcommand{\cE}{{\cal E}}
\newcommand{\bE}{{\mathbf{E}}}
\newcommand{\cG}{{\cal G}}
\newcommand{\cI}{{\cal I}}
\newcommand{\cK}{{\cal K}}
\newcommand{\cX}{{\cal X}}
\newcommand{\cB}{{\cal B}}
\newcommand{\cS}{{\cal S}}
\newcommand{\cM}{{\cal M}}
\newcommand{\cN}{{\cal N}}
\newcommand{\cP}{{\cal P}}
\newcommand{\cO}{{\cal O}}
\newcommand{\cR}{{\cal R}}
\newcommand{\cdb}{\bar{\cal D}}
\newcommand{\ck}{{\cal K}}
\newcommand{\ct}{{\cal T}}
\newcommand{\cV}{{\cal V}}
\newcommand{\bbZ}{\mathbb{Z}}
\newcommand{\bbN}{\mathbb{N}}
\newcommand{\bbR}{\mathbb{R}}
\newcommand{\bbC}{\mathbb{C}}
\newcommand{\bbS}{\mathbb{S}}
\newcommand{\eps}{{\epsilon}}
\newcommand{\inprod}[2]{\left< #1 , #2 \right>}
\newcommand{\inprodt}[2]{\left< #1 , #2 \right>_2}
\newcommand{\inprode}[2]{\left< #1 , #2 \right>_e}
\newcommand{\avg}[1]{\left< #1 \right>}
\newcommand{\expec}[1]{{\cal E}\left\{ #1 \right\}}
\newcommand{\hos}{{\mathbb H}_{os}}
\newcommand{\kraj}{\mbox{\rule{2mm}{2mm}}}
\newcommand{\non}{\nonumber}
\newcommand{\ds}{\displaystyle}
\newcommand{\const}{\mathrm{const.}}
\newcommand{\hxi}{\hat{\xi}}
\newcommand{\heta}{\hat{\eta}}
\newcommand{\hzeta}{\hat{\zeta}}
\newcommand{\hvarsigma}{\hat{\varsigma}}
\newcommand{\hpsi}{\hat{\psi}}
\newcommand{\hphi}{\hat{\phi}}
\newcommand{\hA}{\hat{A}}
\newcommand{\hB}{\hat{B}}
\newcommand{\hC}{\hat{C}}
\newcommand{\hD}{\hat{D}}
\newcommand{\hQ}{\hat{Q}}
\newcommand{\hR}{\hat{R}}
\newcommand{\hP}{\hat{P}}
\newcommand{\hK}{\hat{K}}
\newcommand{\mrd}{\mathrm{d}}
\newcommand{\mre}{\mathrm{e}}
\newcommand{\mri}{\mathrm{i}}
\newcommand{\mrj}{\mathrm{j}}
\newcommand{\bd}{{\bf d}}
\newcommand{\fvec}{{\bf f}}
\newcommand{\bA}{\mathbf{A}}
\newcommand{\bB}{\mathbf{B}}
\newcommand{\bC}{\mathbf{C}}
\newcommand{\bD}{\mathbf{D}}
\newcommand{\bI}{{\bf I}}
\newcommand{\hbd}{{\bf \hat{d}}}
\newcommand{\by}{{\bf y}}
\newcommand{\bx}{{\bf x}}
\newcommand{\bu}{{\bf u}}
\newcommand{\bU}{{\bf U}}
\newcommand{\bF}{{\bf F}}
\newcommand{\bK}{{\bf K}}
\newcommand{\bM}{{\bf M}}
\newcommand{\bN}{{\bf N}}
\newcommand{\bQ}{{\bf Q}}
\newcommand{\bX}{{\bf X}}
\newcommand{\bV}{{\bf V}}
\newcommand{\bPi}{{\bf \Pi}}
\newcommand{\bs}{{\bf s}}
\newcommand{\bphi}{\mbox{\boldmath$\phi$}}
\newcommand{\bpsi}{\mbox{\boldmath$\psi$}}
\newcommand{\bPhi}{\mbox{\boldmath$\Phi$}}
\newcommand{\bPsi}{\mbox{\boldmath$\Psi$}}
\newcommand{\bdelta}{\mbox{\boldmath$\delta$}}
\newcommand{\bnabla}{\mbox{\boldmath$\nabla$}}
\newcommand{\bkappa}{\mbox{\boldmath$\kappa$}}
\newcommand{\bo}{\mbox{\boldmath$\Omega$}}
\newcommand{\bhphi}{\mbox{\boldmath$\hat{\phi}$}}
\newcommand{\bhpsi}{\mbox{\boldmath$\hat{\psi}$}}
\newcommand{\biv}{\textit{\textbf{v}}}
\newcommand{\biu}{\textit{\textbf{u}}}
\newcommand{\mrA}{\mathrm{A}}
\newcommand{\mrB}{\mathrm{B}}
\newcommand{\mrC}{\mathrm{C}}
\newcommand{\mrH}{\mathrm{H}}
\newcommand{\mrT}{\mathrm{T}}
\newcommand{\mrX}{\mathrm{X}}
\newcommand{\mrM}{\mathrm{M}}
\newcommand{\mrU}{\mathrm{U}}
\newcommand{\mrV}{\mathrm{V}}
\newcommand{\mrW}{\mathrm{W}}
\newcommand{\mrY}{\mathrm{Y}}
\newcommand{\mrF}{\mathrm{F}}
\newcommand{\mrG}{\mathrm{G}}
\newcommand{\mrZ}{\mathrm{Z}}
\newcommand{\mrP}{\mathrm{P}}
\newcommand{\mrQ}{\mathrm{Q}}
\newcommand{\mrD}{\mathrm{D}}
\newcommand{\mrN}{\mathrm{N}}
\newcommand{\mrS}{\mathrm{S}}
\newcommand{\G}{\Gamma}
\newcommand{\Dt}{\Delta_\theta}
\newcommand{\invDt}{\Delta_\theta^{-1}}
\newcommand{\Gh}{\hat{G}}
\newcommand{\tp}{{\rm toeplitz}}
\newcommand{\htwo}{{\cal H}_2}
\newcommand{\bY}{\bar{Y}}
\newcommand{\bZ}{\bar{Z}}
\newcommand{\p}{\partial}
\newcommand{\px}{\partial_x}
\newcommand{\py}{\partial_y}
\newcommand{\pz}{\partial_z}
\newcommand{\pt}{\partial_t}
\newcommand{\pyy}{\partial_{yy}}
\newcommand{\pzz}{\partial_{zz}}
\newcommand{\pyz}{\partial_{yz}}
\newcommand{\toep}{\mbox{toep}}
\newcommand{\mrE}{\mathrm{E}}
\newcommand{\bmrE}{\bar{\mathrm{E}}}
\newcommand{\tmrE}{\bar{\mathrm{E}}}
\newcommand{\hmrE}{\hat{\mathrm{E}}}
\newcommand{\hU}{\hat{U}}
\newcommand{\hV}{\hat{V}}
\newcommand{\bAos}{\mathbf{A}_{\rm{os}}}
\newcommand{\bAsq}{\mathbf{A}_{\rm{sq}}}
\newcommand{\bAcp}{\mathbf{A}_{\rm{cp}}}
\newcommand{\lbU}{\overline{\bf {U}}}
\newcommand{\tc}{\textcolor}
\newcommand{\vsp}{\vspace*{0.15cm}}
%----------------------------------------
\newcommand{\DefinedAs}[0]{\mathrel{\mathop:}=}
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\logdet}{log\,det}
\DeclareMathOperator*{\vecform}{vec}
\DeclareMathOperator*{\minimize}{minimize}
\DeclareMathOperator*{\maximize}{maximize}
\DeclareMathOperator*{\subject}{subject~to}
\DeclareMathOperator*{\rank}{rank}

\definecolor{bgblue}{rgb}{0.04,0.19,0.53}
\definecolor{dblue1}{rgb}{0,0.3,0.7}
\definecolor{dred}{rgb}{0.4,0.2,0}

